Towards Improving Reward Design in RL: A Reward Alignment Metric for RL Practitioners

Reinforcement learning agents are fundamentally limited by the quality of the reward functions they learn from, yet reward design is often overlooked under the assumption that a well-defined reward is readily available. However, in practice, designing rewards is difficult, and even when specified, evaluating their correctness is equally problematic: how do we know if a reward function is correctly specified? In our work, we address these challenges by focusing on reward alignment -- assessing whether a reward function accurately encodes the preferences of a human stakeholder. As a concrete measure of reward alignment, we introduce the Trajectory Alignment Coefficient to quantify the similarity between a human stakeholder's ranking of trajectory distributions and those induced by a given reward function. We show that the Trajectory Alignment Coefficient exhibits desirable properties, such as not requiring access to a ground truth reward, invariance to potential-based reward shaping, and applicability to online RL. Additionally, in an 11 -- person user study of RL practitioners, we found that access to the Trajectory Alignment Coefficient during reward selection led to statistically significant improvements. Compared to relying only on reward functions, our metric reduced cognitive workload by 1.5x, was preferred by 82% of users and increased the success rate of selecting reward functions that produced performant policies by 41%.

==> RLC/proofs/proofs_kendall_tau.tex <==
\begin{definition}\label{tac_invariance}
Let \( D_{r, \gamma} \), \( D_{r', \gamma} \), and \( D_h \) be datasets containing preferences over trajectory distributions induced by \( (r, \gamma) \), \( (r', \gamma) \), and by a human, respectively, where \( r' \doteq f(r) \) for some transformation function \( f \).  
The Trajectory Alignment Coefficient ($\sigma_{\textit{TAC}}$) is invariant to \( f \) if:
\[
\sigma_{\text{TAC}}(D_h, D_{r, \gamma}) = \sigma_{\text{TAC}}(D_h, D_{r', \gamma}).
\]
\end{definition}


\begin{theorem}
Consider the infinite-horizon setting, and let \( D_{r, \gamma} \), \( D_{r', \gamma} \), and \( D_h \) be datasets containing preferences over trajectory distributions induced by \( (r, \gamma) \), \( (r', \gamma) \), and by a human, respectively. The Trajectory Alignment Coefficient is invariant to potential-based reward shaping if and only if 
for all corresponding preferences in \( D_{r, \gamma} \), \( D_{r', \gamma} \), \( D_h \), 
 the trajectory distributions \( \eta_i, \eta_j \) being compared belong to the set \(H(\mu)\). 
 \end{theorem}

% \begin{theorem}
% The Trajectory Alignment coefficient is invariant to potential-based reward shaping if and only if for all corresponding pairs of preferences over trajectory distributions,  \( D_r[k] \) and \( D_{r'}[k] \), the trajectory distributions being compared, \( \eta_i, \eta_j \), share the same start state distribution. More specifically, 
% if 
% $\mu_i, \mu_j$ are the start state distributions for \( \eta_i, \eta_j \), then  $\mu_i = \mu_j$. Formally, 
% \begin{gather*}
% \tau(D_{r, \gamma}, D_{r', \gamma}) = 1   
% \iff \; (\mu_i = \mu_j)  \quad \forall \eta_i, \eta_j  \in D_{r, \gamma}, D_{r', \gamma}.
% \end{gather*}
% \end{theorem}





\begin{proof}
Let \( \eta_i, \eta_j  \in D_{r, \gamma}, D_{r', \gamma}\) be arbitrary trajectory distributions, and without loss of generality assume that \( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \). 

By Defintion \eqref{eq:tac} of $\sigma_{\text{TAC}}$, and its invariance property, Definition \eqref{tac_invariance}, 
the stated equivalence holds:
\begin{gather*}
\sigma_{\text{TAC}}(D_h, D_{r, \gamma}) = \sigma_{\text{TAC}}(D_h, D_{r', \gamma}) 
\iff \big(\eta_i \underset{(r, \gamma)}\succ \eta_j \iff \eta_i \underset{(r', \gamma)}\succ \eta_j\big), \; \forall \eta_i, \eta_j \in D_{r, \gamma}, D_{r', \gamma}
\end{gather*}
By Theorem \eqref{potenital_based_reward_shaping_both_cases}, the following biconditional follows:
\begin{gather*}
    \big(\eta_i \underset{(r, \gamma)}\succ \eta_j \iff \eta_i \underset{(r', \gamma)}\succ \eta_j\big) \iff \eta_i, \eta_j \in H(\mu), \; \forall \eta_i, \eta_j \in D_{r, \gamma},D_{r', \gamma}
\end{gather*}
Therefore, we conclude that $\sigma_{\textit{TAC}}$ is invariant to potential-based reward shaping if and only if the trajectory distributions being compared belong to the same set $H(\mu)$.
\begin{gather*}
\sigma_{\text{TAC}}(D_h, D_{r, \gamma}) = \sigma_{\text{TAC}}(D_h, D_{r', \gamma}) \iff \eta_i, \eta_j \in H(\mu), \; \forall \eta_i, \eta_j \in D_{r, \gamma}, D_{r', \gamma}
\end{gather*}
\end{proof}


\begin{theorem}\label{invariant_pos_linear_transformation}
 Given the infinite-horizon setting, the Trajectory Alignment Coefficient is invariant to positive linear transformations. 
\end{theorem}
\begin{proof}
    Let \( \eta_i, \eta_j \in 
    D_{r, \gamma}, D_{r', \gamma}
    \) be arbitrary trajectory distributions, and without loss of generality assume that \( \eta_i^r \succsim \eta_j^r \). From Defintion \eqref{def:preferences_trajectory_distribution}, this implies that
\[
\mathbb{E}_{\tau \sim \eta_i}[G_r(\tau)] \ge \mathbb{E}_{\tau \sim \eta_j}[G_r(\tau)].
\]

We now analyze how the expected return changes under the reward function \( r' \). 
The expected return under the reward function \( r \) is:
\begin{align}
\mathbb{E}_{\tau \sim \eta}[G_r(\tau)] &= \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^t r(s_t, a_t, s_{t+1}) \right]
\end{align}
and the expected return under the shaped reward function \( r' \) is:
\begin{align}
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^t r'(s_t, a_t, s_{t+1}) \right]\label{eq:expected_return_r_prime1}
\end{align}

Substitute \( r'(s, a, s') = \alpha \cdot r(s, a, s') + \beta \) into Equation \eqref{eq:expected_return_r_prime1}, we obtain:
\begin{align*}
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^{\infty} \gamma^t (\alpha \cdot r(s_t, a_t, s_{t+1}) + \beta) \right] \\
&= \alpha \cdot \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^{\infty} \gamma^t r(s_t, a_t, s_{t+1}) \right] + \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^{\infty} \gamma^t \beta \right]
\end{align*}

Since \( \beta \) is a constant, the expectation simplifies as follows:
\begin{align*}
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] &= \alpha \cdot \mathbb{E}_{\tau \sim \eta} [G_r(\tau)] + \beta \sum_{t=0}^{\infty} \gamma^t \\
&= \alpha \cdot \mathbb{E}_{\tau \sim \eta} [G_r(\tau)] + \frac{\beta}{1 - \gamma}
\end{align*}

As $\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)]$ is positive linear transformation of $\mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)]$, we apply Lemma \eqref{linear_transformations_expected_returns_preserves_preferences} to get:
\[\big(\eta_i \underset{(r, \gamma)}\succsim \eta_j \iff \eta_i \underset{(r', \gamma)}\succsim \eta_j\big) \]
Thus, from Equation \eqref{eq:tac} and Definition \eqref{tac_invariance}, we conclude that: \[\sigma_{\text{TAC}}(D_h, D_{r, \gamma}) = \sigma_{\text{TAC}}(D_h, D_{r', \gamma})\] 

\end{proof}
%%%%%%%%%%%%%START OF VERSION 1 OF PROOF TO SHOW TAC IS INVARAINT TO POSITIVE LINEAR TRANSFORMATIONS %%%%%%
% \begin{proof}
% Let \( \eta_i, \eta_j \) be arbitrary trajectory distributions, and without loss of generality assume that \( \eta_i^r \succ \eta_j^r \). From Equation \eqref{eq:stochastic_traj}, this implies that 
% $\mathbb{E}_{\tau\sim\eta_i} [G_r(\tau)] > \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau)]$
% (and vice versa).  

% We now analyze how the expected return changes under the reward function \( r' \), which is a positive linear transformation of \( r \), defined as:
% \[
% r'(s, a, s') \doteq a \cdot r(s, a, s') + b,
% \]
% where \( \alpha > 0 \) and \( \beta \) are constants. The expected returns under \( r \) and \( r' \) are given by Equations \eqref{eq:expected_return_r} and \eqref{eq:expected_return_r_prime}.


% Substituting \( r'(s, a, s') = \alpha \cdot r(s, a, s') + \beta \) into Equation \eqref{eq:expected_return_r_prime}, we obtain:
% \begin{align*}
% \mathbb{E}_{\tau\sim\eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau\sim\eta} \left[ \sum_{t=0}^{\infty} \gamma^t (\alpha \cdot r(s_t, a_t, s_{t+1}) + \beta) \right] \\
% &= \alpha \cdot \mathbb{E}_{\tau\sim\eta} \left[ \sum_{t=0}^{\infty} \gamma^t r(s_t, a_t, s_{t+1}) \right] + \mathbb{E}_{\tau\sim\eta} \left[ \sum_{t=0}^{\infty} \gamma^t \beta \right].
% \end{align*}

% Since \( \beta \) is a constant, the expectation simplifies as follows:
% \begin{align*}
% \mathbb{E}_{\tau\sim\eta}[G_{r'}(\tau)] &= \alpha \cdot \mathbb{E}_{\tau\sim\eta} [G_r(\tau)] + \beta \sum_{t=0}^{\infty} \gamma^t \\
% &= \alpha \cdot \mathbb{E}_{\tau\sim\eta} [G_r(\tau)] + \frac{\beta}{1 - \gamma}.
% \end{align*}

% Since \( \alpha > 0 \), the ordering of expected returns remains unchanged. That is, for all \( \eta_i, \eta_j \in H \),
% \[
% \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau)] > \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau)]
% \implies 
% \mathbb{E}_{\tau\sim\eta_i} [G_{r'}(\tau)] > \mathbb{E}_{\tau\sim\eta_j} [G_{r'}(\tau)].
% \]
% Thus, the preference ordering over trajectory distributions remains unchanged:
% \[
% \eta_i^r \succ \eta_j^r \implies \eta_i^{r'} \succ \eta_j^{r'}.
% \]
% \end{proof}

%%%%%%%%%%%%%END OF VERSION 1 OF PROOF TO SHOW TAC IS INVARAINT TO POSITIVE LINEAR TRANSFORMATIONS %%%%%%

==> RLC/proofs/proofs_reward_shaping.tex <==

% \begin{lemma}\label{constant_diff_same_preferences}
% Given the infinite-horizon setting, if the expected returns under reward function $r'$ is a positive linear transformation of the expected returns under reward function $r$, with respect to all trajectory distributions, then the preference ordering over any two trajectory distributions $\eta_i, \eta_j$ remains unchanged. Formally:
% \[
%  \mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] = \mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)] + \alpha \implies   \Big(\eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff  \eta_i \underset{(r', \gamma)}{\succsim} \eta_j\Big) \;  \forall \eta_i, \eta_j 
% \]
% where the expectations $\mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)]$ and $\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)]$ are taken over the same trajectory distributions.
% \end{lemma}

\begin{lemma}\label{linear_transformations_expected_returns_preserves_preferences}
Given the infinite-horizon setting, if the expected returns under reward function \( r' \) are a positive linear transformation of the expected returns under reward function \( r \), with respect to all trajectory distributions, then the preference ordering over any two trajectory distributions \( \eta_i \) and \( \eta_j \) remains unchanged. Formally:
\[
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] = \alpha \mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)] + \beta \implies 
\Big(\eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff \eta_i \underset{(r', \gamma)}{\succsim} \eta_j\Big) \quad \forall \eta_i, \eta_j,
\]
where \( \alpha > 0 \) and \( \beta \) are constants and the expectations \( \mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)] \) and \( \mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] \) are taken over the same trajectory distributions.
\end{lemma}


% Given the infinite-horizon setting, 
% if reward function \( r' \) is a positive linear transformation of reward function \( r \), then the preference ordering over any two trajectory distributions \( \eta_i, \eta_j \) remains unchanged. 
% Formally:
% \[
% r'(s, a, s') \doteq \alpha \cdot r(s, a, s') + \beta
% \implies   \Big(\eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff  \eta_i \underset{(r', \gamma)}{\succsim} \eta_j\Big) \;  \forall \eta_i, \eta_j
% \]
% where $\alpha > 0$ and $\beta$ are constants.
% \end{lemma}

\begin{proof}
    Let \( \eta_i, \eta_j \) be arbitrary trajectory distributions. Without loss of generality, assume that \mbox{\( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \)}  
    From Definition \ref{def:preferences_trajectory_distribution}, this implies:  
    \[
    \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff \mathbb{E}_{\tau \sim \eta_i}[G_r(\tau)] \geq \mathbb{E}_{\tau \sim \eta_j}[G_r(\tau)]
    \]
    Define the difference in expected returns under \( r \) as:
    \begin{equation}\label{eq:delta_g}
        \Delta_{i,j} \overline{G}(r) \doteq \mathbb{E}_{\tau \sim \eta_i}[G_r(\tau)] - \mathbb{E}_{\tau \sim \eta_j}[G_r(\tau)]
    \end{equation}
    
    Now, consider the transformation of the expected return under \( r' \):
    \[
    \mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] = \alpha \mathbb{E}_{\tau \sim \eta}[G_r(\tau)] + \beta,
    \]
    where \( \alpha > 0 \) and \( \beta \) are constants.  
    Define the corresponding difference under \( r' \):
    \begin{equation}\label{eq:delta_g_prime}
        \Delta_{i,j} \overline{G}(r') = \mathbb{E}_{\tau \sim \eta_i}[G_{r'}(\tau)] - \mathbb{E}_{\tau \sim \eta_j}[G_{r'}(\tau)]
    \end{equation}
    
Substitute the expressions for $\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)]$, we get:
    \[
    \Delta_{i,j} \overline{G}(r') = \Big( \alpha \mathbb{E}_{\tau \sim \eta_i}[G_r(\tau)] + \beta \Big) - \Big( \alpha \mathbb{E}_{\tau \sim \eta_j}[G_r(\tau)] + \beta \Big)
    \]
    Simplify the terms and notice that \( \beta \) cancels out. We obtain:
    \[
    \Delta_{i,j} \overline{G}(r') = \alpha \Delta_{i,j} \overline{G}(r)
    \]

    Now, consider the two cases:

   \textbf{Case 1}: \( \eta_i \underset{(r, \gamma)}{\succ} \eta_j \)
   
     This means \( \Delta_{i,j} \overline{G}(r) > 0 \). Since \( \alpha > 0 \), we have:  
     \[
     \Delta_{i,j} \overline{G}(r') = \alpha \Delta_{i,j} \overline{G}(r) > 0
     \]
     As $\alpha$ is a positive constant, we conclude: \( \eta_i \underset{(r', \gamma)}{\succ} \eta_j \).  

   \textbf{Case 2}: \( \eta_i \underset{(r, \gamma)}{\sim} \eta_j \)
   
     This means \( \Delta_{i,j} \overline{G}(r) = 0 \). Apply the transformation to obtain: 
     \[
     \Delta_{i,j} \overline{G}(r') = \alpha \cdot 0 = 0
     \]
     Thus, \( \eta_i \underset{(r', \gamma)}{\sim} \eta_j \)

    Since both cases preserve the preference ordering, we conclude:
    \[
    \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff \eta_i \underset{(r', \gamma)}{\succsim} \eta_j
    \]
\end{proof}




\begin{lemma}\label{Sufficiency_lemma}[Sufficiency]
    In the infinite horizon setting, if two trajectory distributions \( \eta_i, \eta_j \in H(\mu) \), then potential-based reward shaping preserves their preference ordering with respect to the reward function, $r$, and the potential-based function, $r'$:
    \[
    \eta_i \underset{(r, \gamma)}{\succsim}\eta_j \iff \eta_i \underset{(r', \gamma)}{\succsim} \eta_j.
    \]
    \end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%THIS IS THE START OF VERSION 2 OF THE PROOF FOR THE SUFFICIENCY LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}\label{Sufficiency_lemma_proof}
Let \( \eta_i, \eta_j \in H(\mu)\) be arbitrary trajectory distributions, and without loss of generality assume that \( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \). From Definition \eqref{def:preferences_trajectory_distribution}, this implies that
\[
\mathbb{E}_{\tau \sim \eta_i} [G_r(\tau)] \ge \mathbb{E}_{\tau \sim \eta_j} [G_r(\tau)].
\]
We now analyze how the expected return changes under the potential-based reward function \( r' \).

The expected return under the reward function \( r \) is:
\begin{align}
\mathbb{E}_{\tau \sim \eta}[G_r(\tau)] &= \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^t r(s_t, a_t, s_{t+1}) \right], \label{eq:expected_return_r}
\end{align}
and the expected return under the shaped reward function \( r' \) is:
\begin{align}
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^t r'(s_t, a_t, s_{t+1}) \right]. \label{eq:expected_return_r_prime}
\end{align}

Substitute the definition of the potential-based reward function, Definition \eqref{def:potenital_based_reward_shaping}, into Equation \eqref{eq:expected_return_r_prime}:
\[
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] = \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^t \Big( r(s_t, a_t, s_{t+1}) + \gamma \Phi(s_{t+1}) - \Phi(s_t) \Big) \right].
\]
Distribute $\gamma^t$ and rearrange terms:
\[
\mathbb{E}_{\tau\sim\eta}[G_{r'}(\tau)] = \mathbb{E}_{\tau\sim \eta} \left[ \sum_{t=0}^\infty \gamma^t  r(s_t, a_t, s_{t+1}) + \gamma^t \gamma\Phi(s_{t+1}) - \gamma^t \Phi(s_t)  \right] 
\]
\[
\begin{aligned}
    &= \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^t r(s_t, a_t, s_{t+1}) \right] 
    + \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=0}^\infty \gamma^{t+1} \Phi(s_{t+1}) - \gamma^t \Phi(s_t) \right] \\
    &= \mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)] + \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=1}^\infty \gamma^{t} \Phi(s_t) - \sum_{t=0}^\infty \gamma^t \Phi(s_t) \right]
\end{aligned}
\]
Split $\sum_{t=0}^\infty \gamma^t \Phi(s_t)$ into two parts, one from $t=1$ to $\infty$ and the other isolating $t=0$:
\[
     =\mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)] + \mathbb{E}_{\tau \sim \eta} \left[ \sum_{t=1}^\infty \gamma^{t} \Phi(s_t) - \sum_{t=1}^\infty \gamma^t \Phi(s_t) - \gamma^0 \Phi(s_0) \right] 
\]
Now, combine like-terms and $\sum_{t=1}^\infty \gamma^{t} \Phi(s_t)$ gets canceled out:
\[
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] = \mathbb{E}_{\tau \sim \eta}[G_r(\tau)] - \mathbb{E}_{\tau \sim \eta} \left[ \Phi(s_0) \right]
\]
As \( \Phi(s_0) \) depends only on the start-state distribution \( \mu \), and \( \mu \) is the same for all \( \eta \in H(\mu) \), we conclude that the expected returns under \( r \) and \( r' \) differ by a constant,
$\mathbb{E}_{s_{0}\sim \mu} \left[\Phi(s_0) \right]$:
\begin{equation}
\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)] = \mathbb{E}_{\tau \sim \eta}[G_r(\tau)] - \mathbb{E}_{s_0 \sim \mu} \left[ \Phi(s_0) \right] \label{eq:shaping_expected_return_with_phi}
\end{equation}

As $\mathbb{E}_{\tau \sim \eta}[G_{r'}(\tau)]$ is a positive linear transformation of $\mathbb{E}_{\tau \sim \eta}[G_{r}(\tau)]$, we apply Lemma \ref{linear_transformations_expected_returns_preserves_preferences} and conclude that the preference remains unchanged under reward shaping:
\[
\eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff \eta_i \underset{(r', \gamma)}{\succsim} \eta_j \; \forall \eta_i, \eta_j \in H(\mu)
\]
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%THIS IS THE END OF VERSION 2 OF THE PROOF FOR THE SUFFICIENCY LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{lemma}\label{Necessity_lemma}[Necessity]
   In the infinite horizon setting, if two trajectory distributions \( \eta_i \in H(\mu_i) \) and \( \eta_j \in H(\mu_j) \) have different start-state distributions (\(\mu_i \neq \mu_j\)), then there exists a potential function \( \Phi \) such that:
    \[
    \eta_i \underset{(r, \gamma)}{\succsim}  \eta_j \iff \eta_i \underset{(r', \gamma)}{\prec} \eta_j.
    \]
    \end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%THIS IS THE Start OF VERSION 2 OF THE PROOF FOR THE Necessity LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}\label{Necessity_lemma_proof}
Let \( \eta_i \in H(\mu_i) \) and \( \eta_j \in H(\mu_j) \)
be arbitrary trajectory distributions that have different start-state distributions (\(\mu_i \neq \mu_j\)). Without loss of generality assume that \( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \).  From Definition \eqref{def:preferences_trajectory_distribution}, this implies that: 
\[\mathbb{E}_{\tau\sim\eta_i} [G_r(\tau)] \ge \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau)]\] We now analyze how the expected return changes under the potential-shaped reward function \( r' \). 

From Equation \eqref{eq:shaping_expected_return_with_phi} we have
\begin{align}
\mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r'}] &= 
\mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - 
\mathbb{E}_{s_{0}\sim \mu_{i}} \left[\Phi(s_0) \right], \label{eq:expected_return_phii} \\
\mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r'}] &= 
\mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)] - 
\mathbb{E}_{s_{0}\sim \mu_{j}} \left[\Phi(s_0) \right]. \label{eq:expected_return_phij}
\end{align}
Next, we define $\Delta_{i,j} \overline{G}(r), \Delta_{i,j} \overline{G}(r')$:
\begin{equation}\label{eq:delta_g2}
\Delta_{i,j} \overline{G}(r) \doteq \mathbb{E}_{\tau \sim \eta_i}[G_r(\tau)] - \mathbb{E}_{\tau \sim \eta_j}[G_r(\tau)]
\end{equation}
\begin{equation}\label{eq:delta_g_prime2}
\Delta_{i,j} \overline{G}(r) \doteq \mathbb{E}_{\tau \sim \eta_i}[G_{r'}(\tau)] - \mathbb{E}_{\tau \sim \eta_j}[G_{r'}(\tau)]
\end{equation}
Substitute Equations \eqref{eq:expected_return_phii} and \eqref{eq:expected_return_phij} into Equation \eqref{eq:delta_g_prime2} to obtain $\Delta_{i,j} \overline{G}(r')$:
\begin{align*}
\Delta_{i,j} \overline{G}(r') 
&= \Bigl(
\mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] -  \mathbb{E}_{s_{0}\sim \mu_{i}}\left[\Phi(s_0)\right]\Bigr) - \Bigl(
\mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)] - 
\mathbb{E}_{s_{0}\sim \mu_{j}}\left[\Phi(s_0)\right]
\Bigr)
\end{align*}

Rearrange terms and substitute in the equation for $\Delta_{i,j} \overline{G}(r)$, Equation \eqref{eq:delta_g2}:
\begin{align}
\Delta_{i,j} \overline{G}(r') &= \Bigl(\mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)]\Bigr) - \Bigl(\mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]  - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]\Bigr) \nonumber \\
&= \Delta_{i,j} \overline{G}(r) - \Bigl(\mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]  - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]\Bigr)\label{eq:delta_g_with_phi}
\end{align}
Now we show that there exists a potential-based shaping function that will invert the preference ordering over trajectory distributions $\eta_i, \eta_j$, that is $ \exists \Phi: \mathcal{S} \to \mathbb{R}$ such that \( \eta_i \underset{(r', \gamma)}{\prec} \eta_j\).

From Definition \ref{def:preferences_trajectory_distribution}, it follows that:
\begin{align}
 \eta_i \underset{(r', \gamma)}{\prec} \eta_j \iff \Delta_{i,j} \overline{G}(r') < 0 \nonumber
\end{align}
This provides the necessary condition for the existence of such a shaping function. Now let $\Delta_{i,j}\overline{\Phi}$ be defined as:
\begin{equation}\label{delta_phi}
\Delta_{i,j}\overline{\Phi} \doteq \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]
\end{equation}

Combine Equations \eqref{eq:delta_g_with_phi} and \eqref{delta_phi} to get:
\begin{equation}
    \Delta_{i,j} \overline{G}(r') = \Delta_{i,j} \overline{G}(r) - \Delta_{i,j}\overline{\Phi}  \nonumber
\end{equation}
where $\Delta_{i,j} \overline{G}(r) > 0$, since \( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \). Now it is clear that: \begin{equation}
    \Delta_{i,j} \overline{G}(r') < 0 \iff \Delta_{i,j}\overline{\Phi} > \Delta_{i,j} \overline{G}(r)  \nonumber
\end{equation}

We now provide an example of a potential-based shaping function for which $\Delta_{i,j}\overline{\Phi} > \Delta_{i,j} \overline{G}(r)$.
To begin, let us partition the state space $\mathcal{S}$ into two subsets: (1) the set of states that are more probable under $\mu_i$ and (2) those that are more probable under $\mu_j$, denoted as $\mathcal{S}_{\mu_i > \mu_j}$ and $\mathcal{S}_{\mu_i \leq \mu_j}$, respectively:
\begin{align}
    \mathcal{S}_{\mu_i > \mu_j} &= \{s|s\in\mathcal{S}, \mu_i(s)>\mu_j(s)\}\label{eq:partition_ui_greater_uj} \\
    \mathcal{S}_{\mu_i \leq \mu_j} &= \{s|s\in\mathcal{S}, \mu_i(s)\leq\mu_j(s)\}\label{eq:partition_ui_lesser_uj}
\end{align}
Next, we define the potential-based shaping function $\Phi: \mathcal{S} \to \mathbb{R}$ as a piecewise function, which takes the following form:
\begin{equation}\label{eq:peicewise_function}
    \Phi(s) =
\begin{cases} 
\frac{\Delta_{i,j} \overline{G}(r) + \epsilon}{\int_{s\in\mathcal{S}_{\mu_i>\mu_j}}\mu_i(s)-\mu_j(s)}, & \text{if } s\in\mathcal{S}_{\mu_i>\mu_j} \\
0 & \text{if } s\in\mathcal{S}_{\mu_i\leq\mu_j} 
\end{cases}
\end{equation}
where $\epsilon\in\mathbb{R}, \epsilon > 0$. For this shaping function, we define the difference in expected values as:
\begin{align*}
    \Delta_{i,j}\overline{\Phi} &\doteq \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right] 
\end{align*}
We can express the expectation in integral form and rearrange the terms:
\begin{align*}
    &= \int_{s\in\mathcal{S}}\mu_i(s)\Phi(s) - \int_{s\in\mathcal{S}}\mu_j(s)\Phi(s) \\
    &= \int_{s\in\mathcal{S}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) 
\end{align*}
Decompose the integral over the two partitions defined in Equations \eqref{eq:partition_ui_greater_uj} and \eqref{eq:partition_ui_lesser_uj}. Notice that $ \int_{s\in\mathcal{S}_{\mu_i \leq \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s)$ goes to $0$ by Equation \eqref{eq:peicewise_function}:
\begin{align*}
    &= \int_{s\in\mathcal{S}_{\mu_i > \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) + \int_{s\in\mathcal{S}_{\mu_i \leq \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) \\
    &= \int_{s\in\mathcal{S}_{\mu_i > \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) 
\end{align*}
Move $\Phi(s)$ outside of the integral as it is a constant by Equation \eqref{eq:peicewise_function} and simplify:
\begin{align*}
    &= \frac{\Delta_{i,j} \overline{G}(r) + \epsilon}{\int_{s\in\mathcal{S}_{\mu_i>\mu_j}}\mu_i(s)-\mu_j(s)} \int_{s\in\mathcal{S}_{\mu_i > \mu_j}}\mu_i(s) - \mu_j(s) \\
    &= \Delta_{i,j} \overline{G}(r) + \epsilon
\end{align*}
Hence $\Delta_{i,j}\overline{\Phi} = \Delta_{i,j} \overline{G}(r) + \epsilon > \Delta_{i,j} \overline{G}(r)$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%THIS IS THE end OF VERSION 2 OF THE PROOF FOR THE Necessity LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{potenital_based_reward_shaping_both_cases}

In the infinite-horizon setting, let $(r,\gamma)$ and two trajectory distributions \( \eta_i \in H(\mu_i) \) and \( \eta_j \in H(\mu_j) \) be given. Potential-based reward shaping \( r' \) maintains the preference ordering over all trajectory distributions if and only if \( \mu_i = \mu_j \).
Formally,  
\[
\eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff \eta_i \underset{(r', \gamma)}{\succsim} \eta_j \quad \forall \eta_i \in H(\mu_i), \eta_j \in H(\mu_j) \text{ such that } \mu_i = \mu_j.
\] 
\end{theorem}
The proof of Theorem \ref{potenital_based_reward_shaping_both_cases} follows directly from Lemmas \ref{Sufficiency_lemma} and \ref{Necessity_lemma}. 
% %%%%%%%%%%%%%%%%%%%%%%% THIS IS START OF VERISON 1 OF THE PROOF FOR THE Sufficiency LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}\label{Sufficiency_lemma_proof}
% \textbf{Sufficiency Lemma.}
% Let \( \eta_i, \eta_j \in H(\mu)\) be arbitrary trajectory distributions, and without loss of generality assume that $\eta_i \underset{(r, \gamma)}{\succsim} \eta_j$.  From Equation \eqref{eq:stochastic_traj}, this implies that $\mathbb{E}_{\tau\sim\eta_i} [G_r(\tau)] \ge \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau)]$.  
% We now analyze how the expected return changes under the potential-based reward function \( r' \). 
% % The definition of \( \mathbb{E}_{\tau\sim \eta}[G_{r}(\tau)]  \) and \( \mathbb{E}_{\tau\sim \eta}[G_{r'}(\tau)]  \) are as follows:
% \begin{align}
% \mathbb{E}_{\tau\sim \eta}[G_{r}(\tau)] &\doteq \mathbb{E}_{\tau\sim \eta}\left[ \sum_{t=0}^\infty \gamma^t r(s_t, a_t, s_{t+1}) \right], \label{eq:expected_return_r} \\
% \mathbb{E}_{\tau\sim \eta}[G_{r'}(\tau)] &\doteq  \mathbb{E}_{\tau\sim \eta}\left[ \sum_{t=0}^\infty \gamma^t r'(s_t, a_t, s_{t+1}) \right]. \label{eq:expected_return_r_prime}
% \end{align}

% Substitute the definition of the potential-based reward function, Definition \ref{def:potenital_based_reward_shaping}, into Equation \eqref{eq:expected_return_r_prime} and rewrite $\mathbb{E}_{\tau\sim \eta}[G_{r'}(\tau)]$:
% \begin{align*}
% \mathbb{E}_{\tau\sim\eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau\sim\eta} \left[ \sum_{t=0}^{\infty} \gamma^t \Bigl(r(s_t, a_t, s_{t+1}) + \gamma \Phi(s_{t+1}) - \Phi(s_t)\Bigr) \right].
% \end{align*}

% Expand the summation and rearrange terms:
% \begin{align}
% \mathbb{E}_{\tau\sim\eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau\sim \eta} \left[ \sum_{t=0}^\infty \gamma^t  r(s_t, a_t, s_{t+1}) + \gamma^t \gamma\Phi(s_{t+1}) - \gamma^t \Phi(s_t)  \right] \nonumber\\
% &= \mathbb{E}_{\tau\sim \eta} \left[ \sum_{t=0}^\infty \gamma^t  r(s_t, a_t, s_{t+1})\right] + \mathbb{E}_{\tau\sim \eta} \left[ \sum_{t=0}^\infty \gamma^{t+1}\Phi(s_{t+1}) - \gamma^t \Phi(s_t)  \right] \nonumber\\
% &= \mathbb{E}_{\tau\sim \eta}[G_{r}(\tau)] + \mathbb{E}_{\tau\sim \eta} \left[ \sum_{t=1}^\infty \gamma^{t}\Phi(s_{t}) - \sum_{t=0}^\infty \gamma^t \Phi(s_t)  \right] \nonumber\\
% &= \mathbb{E}_{\tau\sim \eta}[G_{r}(\tau)] + \mathbb{E}_{\tau\sim \eta} \left[ \sum_{t=1}^\infty \gamma^{t}\Phi(s_{t}) - \sum_{t=1}^\infty \gamma^t \Phi(s_t) - \gamma^{0}\Phi(s_0)  \right] \nonumber\\
% &= \mathbb{E}_{\tau\sim \eta}[G_{r}(\tau)] - \mathbb{E}_{\tau\sim \eta} \left[ \Phi(s_0) \right] \nonumber\\
% \mathbb{E}_{\tau\sim\eta}[G_{r'}(\tau)] &= \mathbb{E}_{\tau\sim \eta}[G_{r}(\tau)] - \mathbb{E}_{s_{0}\sim \mu} \left[\Phi(s_0) \right]. \label{eq:shaping_expected_return}
% \end{align}

% As \( \Phi(s_0) \) depends only on the start-state distribution \( \mu \), and \( \mu \) is the same for all \( \eta \in H(\mu) \), we conclude that the expected returns under \( r \) and \( r' \) differ by a constant,
% $\mathbb{E}_{s_{0}\sim \mu} \left[\Phi(s_0) \right]$.

% Let us denote the difference in expected return (under reward function $r$) for two trajectory distributions as $\Delta_{i,j} \overline{G}(r)$:
% \begin{equation}
% \Delta_{i,j} \overline{G}(r) \doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)]  \label{eq:delta_g}
% \end{equation}
% Note: it follows from definition \ref{def:preferences_trajectory_distribution} that $\eta_i \underset{(r, \gamma)}{\succsim} \eta_j$ if and only if $\Delta_{i,j} \overline{G}(r)\geq 0$.
% % Note: it follows from definition \ref{def:preferences_trajectory_distribution} that $\eta_i \succsim_r \eta_j$ if and only if $\Delta_{i,j} \overline{G}(r)\geq 0$.
% % Note: it follows from definition \ref{def:preferences_trajectory_distribution} that $\eta_i \succsim^r \eta_j$ if and only if $\Delta_{i,j} \overline{G}(r)\geq 0$.

% Given equation \eqref{eq:shaping_expected_return}, we have
% \begin{align}
%     \Delta_{i,j} \overline{G}(r') &= \mathbb{E}_{\tau\sim \eta_i}[G_{r'}(\tau)] - \mathbb{E}_{\tau\sim \eta_j}[G_{r'}(\tau)] \nonumber\\
%     &= \Bigl(\mathbb{E}_{\tau\sim \eta_i}[G_{r}(\tau)] - \mathbb{E}_{s_{0}\sim \mu} \left[\Phi(s_0) \right]\Bigr) - \Bigl(\mathbb{E}_{\tau\sim \eta_j}[G_{r}(\tau)] - \mathbb{E}_{s_{0}\sim \mu} \left[\Phi(s_0) \right]\Bigr) \label{eq:same_mu}\\
%     &= \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)] \nonumber\\
%     \Delta_{i,j} \overline{G}(r') &= \Delta_{i,j} \overline{G}(r)
% \end{align}
% where in equation \eqref{eq:same_mu} we use the result from equation \eqref{eq:shaping_expected_return}, and the fact that $\eta_i, \eta_j$ share the same initial state distribution $\mu$ (i.e., $\eta_i, \eta_j \in H(\mu)$).

% Therefore, if 
% \begin{enumerate}[leftmargin=3em]
%     \item $\eta_i, \eta_j \in H(\mu)$,
%     \item $r'(s, a, s') = r(s,a,s') + \gamma \Phi(s') - \Phi(s)$, and
%     \item $\eta_i \underset{(r, \gamma)}{\succsim} \eta_j$,
% \end{enumerate}
% then $\Delta_{i,j} \overline{G}(r') = \Delta_{i,j} \overline{G}(r) \geq 0$, and we have $\eta_i \underset{(r', \gamma)}{\succsim }\eta_j$. 
% The preference remains unchanged under reward shaping:
% \[
% \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \iff \eta_i \underset{(r', \gamma)}{\succsim }\eta_j.
% \]
% for all \mbox{$\eta_i, \eta_j \in H(\mu)$}.
% \end{proof}

    % %%%%%%%%%%%%%%%%%%%%%%% THIS IS END OF VERISON 1 OF THE PROOF FOR THE Sufficiency LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%





    % %%%%%%%%%%%%%%%%%%%%%%% THIS IS START OF VERISON 1 OF THE PROOF FOR THE Necessity LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  \begin{proof}\label{Necessity_lemma_proof}
% \textbf{Necessary Lemma.}
% Let \( \eta_i \in H(\mu_i) \) and \( \eta_j \in H(\mu_j) \)
% be arbitrary trajectory distributions that have different start-state distributions (\(\mu_i \neq \mu_j\)). Without loss of generality assume that \( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \). From Equation \eqref{eq:stochastic_traj}, this implies that
% $\mathbb{E}_{\tau\sim\eta_i} [G_r(\tau)] \ge \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau)]$. We now analyze how the expected return changes under the potential-shaped reward function \( r' \). 
% % Let:
% % \begin{align}
% % \Delta_{i,j} \langle G_r \rangle &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)]\\ 
% % \Delta_{i,j} \langle G(r) \rangle &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)]\\ 
% % \Delta_{i,j} \langle G \rangle (r) &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)]\\ 
% % \Delta_{i,j} \overline{G}_r &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)] \\
% % \Delta_{i,j} \overline{G}(r) &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)] \\
% % \Delta_{i,j} \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)] \\
% % \Delta_{i,j} \mathbb{E} [G_r] &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)] 
% % \end{align}

% From Equation \eqref{eq:shaping_expected_return_with_phi}, we have
% \begin{align}
% \mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r'}] &= 
% \mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{i}} \left[\Phi(s_0) \right], \label{eq:expected_return_phii} \\
% \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r'}] &= 
% \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{j}} \left[\Phi(s_0) \right]. \label{eq:expected_return_phij}
% \end{align}

% Substitute Equations \eqref{eq:expected_return_phii} and \eqref{eq:expected_return_phij} into Equation \eqref{eq:delta_g} to obtain $\Delta_{i,j} \overline{G}(r')$:
% \begin{align*}
% \Delta_{i,j} \overline{G}(r') &= 
% \Bigl(
% \mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{i}}\left[\Phi(s_0)\right]
% \Bigr) \\
% &\quad - \Bigl(
% \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{j}}\left[\Phi(s_0)\right]
% \Bigr)
% \end{align*}

% Rearrange terms:
% \begin{align*}
% \Delta_{i,j} \overline{G}(r') &= \Bigl(\mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)]\Bigr) - \Bigl(\mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]  - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]\Bigr)\\
% % &= \Delta G_{r} -
% % \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] + \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]
% &= \Delta_{i,j} \overline{G}(r) - \Bigl(\mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]  - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]\Bigr)
% \end{align*}


% % Suppose we choose a potential function, $\Phi$, such that \bk{I was only able to skim this proof. Consider explicitly defining $\Phi$ as part of the proof as a function of the two distributions, if you can.}:
% % \begin{align*}
% %     &\mathbb{E}_{s_{0}\sim \mu_i} \left[\Phi(s_0) \right] - \mathbb{E}_{s_{0}\sim \mu_j} \left[\Phi(s_0) \right]  > \Delta G_{r} \\
% % %     &\mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right] -
% % % \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]  < -\Delta G_{r} \\
% %     &\implies \Delta G_{r'}  < 0 \\
% %     &\implies \mathbb{E}_{\tau\sim\eta_i} [G_{r'}(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_{r'}(\tau_j)] < 0 \\
% %     &\implies \mathbb{E}_{\tau\sim\eta_i} [G_{r'}(\tau_i)] < \mathbb{E}_{\tau\sim\eta_j} [G_{r'}(\tau_j)] \\
% %     &\implies \eta_i \underset{(r', \gamma)}{\prec} \eta_j
% % \end{align*}
% Now we show that there exists a potential-based shaping function $\Phi: \mathcal{S} \to \mathbb{R}$ such that \( \eta_i \underset{(r, \gamma)}{\prec} \eta_j\). That is, there exists a potential-based shaping function that will invert the preference ordering over trajectory distributions $\eta_i, \eta_j$.

% It follows from definition \ref{def:preferences_trajectory_distribution} that
% \begin{equation}
%  \eta_i \underset{(r, \gamma)}{\prec} \eta_j \iff \Delta_{i,j} \overline{G}(r') < 0.
% \end{equation}
% Let $\Delta_{i,j}\overline{\Phi} \doteq \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]$. Then we have
% \begin{equation}
%     \Delta_{i,j} \overline{G}(r') = \Delta_{i,j} \overline{G}(r) - \Delta_{i,j}\overline{\Phi}
% \end{equation}
% where $\Delta_{i,j} \overline{G}(r) > 0$, since \( \eta_i \underset{(r, \gamma)}{\succsim} \eta_j \). Now it is clear that \begin{equation}
%     \Delta_{i,j} \overline{G}(r') < 0 \iff \Delta_{i,j}\overline{\Phi} > \Delta_{i,j} \overline{G}(r).
% \end{equation}

% We now give an example of a potential-based shaping function for which $\Delta_{i,j}\overline{\Phi} > \Delta_{i,j} \overline{G}(r)$.

% Let us partition the state space $\mathcal{S}$ into the set of states that are more probable under $\mu_i$ and those that are more probable under $\mu_j$, denoted as $\mathcal{S}_{\mu_i > \mu_j}$ and $\mathcal{S}_{\mu_i \leq \mu_j}$, respectively:
% \begin{align}
%     \mathcal{S}_{\mu_i > \mu_j} &= \{s|s\in\mathcal{S}, \mu_i(s)>\mu_j(s)\} \\
%     \mathcal{S}_{\mu_i \leq \mu_j} &= \{s|s\in\mathcal{S}, \mu_i(s)\leq\mu_j(s)\}
% \end{align}
% Let the potential-based shaping function $\Phi: \mathcal{S} \to \mathbb{R}$ be defined as the following piecewise function.
% \begin{equation}
%     \Phi(s) =
% \begin{cases} 
% 0, & \text{if } s\in\mathcal{S}_{\mu_i\leq\mu_j} \\ 
% \frac{\Delta_{i,j} \overline{G}(r) + \epsilon}{\int_{s\in\mathcal{S}_{\mu_i>\mu_j}}\mu_i(s)-\mu_j(s)}, & \text{if } s\in\mathcal{S}_{\mu_i>\mu_j}
% \end{cases}
% \end{equation}
% where $\epsilon\in\mathbb{R}, \epsilon > 0$. For this shaping function, we have:
% \begin{align}
%     \Delta_{i,j}\overline{\Phi} &\doteq \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] - \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right] \\
%     &= \int_{s\in\mathcal{S}}\mu_i(s)\Phi(s) - \int_{s\in\mathcal{S}}\mu_j(s)\Phi(s) \\
%     &= \int_{s\in\mathcal{S}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) \\
%     &= \int_{s\in\mathcal{S}_{\mu_i > \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) + \int_{s\in\mathcal{S}_{\mu_i \leq \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) \\
%     &= \int_{s\in\mathcal{S}_{\mu_i > \mu_j}}\bigl(\mu_i(s) - \mu_j(s)\bigr)\Phi(s) \\
%     &= \frac{\Delta_{i,j} \overline{G}(r) + \epsilon}{\int_{s\in\mathcal{S}_{\mu_i>\mu_j}}\mu_i(s)-\mu_j(s)} \int_{s\in\mathcal{S}_{\mu_i > \mu_j}}\mu_i(s) - \mu_j(s) \\
%     &= \Delta_{i,j} \overline{G}(r) + \epsilon
% \end{align}
% Hence $\Delta_{i,j}\overline{\Phi} = \Delta_{i,j} \overline{G}(r) + \epsilon > \Delta_{i,j} \overline{G}(r)$.
% \end{proof}

    % %%%%%%%%%%%%%%%%%%%%%%% THIS IS END OF VERISON 1 OF THE PROOF FOR THE Necessity LEMMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%IGNORE WHAT IS BELOW%%%%%%%%%%%%%%

% \begin{proof}

% Assume the infinite horizon setting. Let \( \eta_i, \eta_j \) be arbitrary trajectory distributions, and without loss of generality assume that under reward function \( r \), \( \eta_i^r \succ \eta_j^r \). This implies that
% $\mathbb{E}_{\tau\sim\eta_i} [G_r(\tau)] > \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau)]$. We now analyze how the expected return changes under the potential-based reward function \( r' \). Let:
% \begin{align}
% \Delta G_r &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_r(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_r(\tau_j)] 
% \implies \Delta G_r  > 0, \label{eq:delta_gr} \\
% \Delta G_{r'} &\doteq \mathbb{E}_{\tau\sim\eta_i} [G_{r'}(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_{r'}(\tau_j)]. \label{eq:delta_gr_prime}
% \end{align}


% From Theorem \ref{Sufficiency_for_invariance}, we have
% \begin{align}
% \mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r'}] &= 
% \mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{i}} \left[\Phi(s_0) \right], \label{eq:expected_return_phii} \\
% \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r'}] &= 
% \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{j}} \left[\Phi(s_0) \right]. \label{eq:expected_return_phij}
% \end{align}

% Substitute Equations \ref{eq:expected_return_phii} and \ref{eq:expected_return_phij} into Equation \ref{eq:delta_gr_prime} and rewrite $\Delta G_{r'}$:
% \begin{align*}
% \Delta G_{r'} &= 
% \left[
% \mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{i}}\left[\Phi(s_0)\right]
% \right] \\
% &\quad - \left[
% \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)] - 
% \mathbb{E}_{s_{0}\sim \mu_{j}}\left[\Phi(s_0)\right]
% \right]
% \end{align*}

% Rearrange terms:
% \begin{align*}
% \Delta G_{r'} &= \left(\mathbb{E}_{\tau\sim \eta_{i}(\tau)}[G_{r}(\tau)] - \mathbb{E}_{\tau\sim \eta_{j}(\tau)}[G_{r}(\tau)]\right)  \\
% &\quad - \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] + \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right] \\
% &= \Delta G_{r} -
% \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right] + \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right]
% % &= \Delta G_{r} + \mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right] -
% % \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]
% \end{align*}


% Suppose we choose a potential function, $\Phi$, such that \bk{I was only able to skim this proof. Consider explicitly defining $\Phi$ as part of the proof as a function of the two distributions, if you can.}:
% \begin{align*}
%     &\mathbb{E}_{s_{0}\sim \mu_i} \left[\Phi(s_0) \right] - \mathbb{E}_{s_{0}\sim \mu_j} \left[\Phi(s_0) \right]  > \Delta G_{r} \\
% %     &\mathbb{E}_{s_{0}\sim \mu_j}\left[\Phi(s_0)\right] -
% % \mathbb{E}_{s_{0}\sim \mu_i}\left[\Phi(s_0)\right]  < -\Delta G_{r} \\
%     &\implies \Delta G_{r'}  < 0 \\
%     &\implies \mathbb{E}_{\tau\sim\eta_i} [G_{r'}(\tau_i)] - \mathbb{E}_{\tau\sim\eta_j} [G_{r'}(\tau_j)] < 0 \\
%     &\implies \mathbb{E}_{\tau\sim\eta_i} [G_{r'}(\tau_i)] < \mathbb{E}_{\tau\sim\eta_j} [G_{r'}(\tau_j)] \\
%     &\implies \eta_i^{r'} \prec \eta_j^{r'}
% \end{align*}
% \end{proof}


